QuasiNav: Asymmetric Cost-Aware Navigation Planning with Constrained Quasimetric Reinforcement Learning

Autonomous navigation in unstructured outdoor environments is inherently challenging due to the presence of asymmetric traversal costs, such as varying energy expenditures for uphill versus downhill movement. Traditional reinforcement learning methods often assume symmetric costs, which can lead to suboptimal navigation paths and increased safety risks in real-world scenarios. In this paper, we introduce QuasiNav, a novel reinforcement learning framework that integrates quasimetric embeddings to explicitly model asymmetric costs and guide efficient, safe navigation. QuasiNav formulates the navigation problem as a constrained Markov decision process (CMDP) and employs quasimetric embeddings to capture directionally dependent costs, allowing for a more accurate representation of the terrain. This approach is combined with adaptive constraint tightening within a constrained policy optimization framework to dynamically enforce safety constraints during learning. We validate QuasiNav across three challenging navigation scenarios-undulating terrains, asymmetric hill traversal, and directionally dependent terrain traversal-demonstrating its effectiveness in both simulated and real-world environments. Experimental results show that QuasiNav significantly outperforms conventional methods, achieving higher success rates, improved energy efficiency, and better adherence to safety constraints.

==> Sections/Experiments_and_Results.tex <==
\section{Experiments and Results}

We conduct a comprehensive evaluation of QCPO against a wide range of baselines, addressing the reviewers' concerns about fair comparisons and the necessity of our approach. We compare QCPO with state-of-the-art reinforcement learning algorithms: Trust Region Policy Optimization (TRPO) \cite{schulman2015trust}, Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, Soft Actor-Critic (SAC) \cite{haarnoja2018soft}, and Constrained Policy Optimization (CPO) \cite{achiam2017constrained}. As per the reviewers' suggestions, we also include comparisons with safety-aware RL methods: Safety-Aware Reinforcement Learning (SARL) \cite{garcia2015comprehensive}. Additionally, we compare against classical navigation methods: Dynamic Window Approach (DWA) \cite{fox1997dynamic}.

All learning-based algorithms use identical neural network architectures and hyperparameters where applicable. Our implementation uses PyTorch and integrates with ROS Noetic. We use the Unity simulator with a high-fidelity model of the Clearpath Jackal UGV, incorporating diverse terrains and elevations within a 100m × 100m region for training. The Unity simulation environment incorporates diverse terrains and elevations for training and testing. The real and simulated testing were conducted in different outdoor scenarios. Particularly, the real-world environments differ significantly in terms of terrain structure (i.e., elevation gradient) and surface properties (i.e., grass and tiny gravel regions with different levels of friction) which are not fully captured in the simulator. For safety, we limit the maximum elevation gain to ~3m in real-world tests, compared to ~4m in simulations.


\subsection{Navigation Scenarios}

To rigorously evaluate QCPO's performance, we designed three challenging scenarios that specifically highlight asymmetric and direction-dependent traversal costs:

\begin{enumerate}
    \item \textbf{Undulating Terrain Navigation:} A 100m × 100m area with slopes ranging from 0° to 30° and varying soil types (grass, gravel, sand).
    \item \textbf{Hill Traversal with Asymmetric Costs:} An 80m × 80m area featuring a central hill with 20° slopes and different surface conditions on each side.
    \item \textbf{Directionally Dependent Terrain Traversal:} A 120m × 120m area with four distinct terrain types, each with direction-dependent traversal properties.
\end{enumerate}

\subsection{Implementation Details}

To ensure fair comparison, as requested by the reviewers, we implement safety constraints for all algorithms, including those not originally designed for constrained MDPs. For unconstrained algorithms (TRPO, PPO, SAC), we use a Lagrangian relaxation method to incorporate safety constraints. We use identical constraint formulations across all algorithms. The state space includes the robot's position, orientation, linear and angular velocities, and processed LiDAR features. The action space consists of continuous linear and angular velocity commands. We train each algorithm for 2 million timesteps across 10 random seeds to ensure statistical significance.

\subsection{Results and Analysis}

Table \ref{tab:nav_performance} presents a comprehensive comparison of navigation performance across all scenarios, averaged over 100 test episodes for each algorithm.

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt} % Reduce horizontal padding
\resizebox{\columnwidth}{!}{ % Resize to fit column width
\begin{tabular}{lccccccc}
\hline
\textbf{Metric} & \textbf{QCPO} & \textbf{CPO} & \textbf{SARL} & \textbf{PPO} & \textbf{TRPO} & \textbf{SAC} & \textbf{DWA} \\
\hline
\textbf{Success Rate (\%)} & \textbf{94.7} & 82.3 & 80.5 & 75.1 & 73.8 & 71.5 & 88.9 \\
\textbf{Path Efficiency} & \textbf{1.12} & 1.25 & 1.28 & 1.38 & 1.41 & 1.33 & 1.18 \\
\textbf{Energy Efficiency (J/m)} & \textbf{142.6} & 178.3 & 182.7 & 195.7 & 201.4 & 189.6 & 172.1 \\
\textbf{Safety Violation Rate (\%)} & \textbf{2.1} & 4.8 & 4.5 & 7.2 & 7.6 & 6.3 & 5.2 \\
\textbf{Sample Efficiency (×10\textsuperscript{3} steps)} & \textbf{450} & 620 & 635 & 780 & 810 & 710 & N/A \\
\hline
\end{tabular}}
\caption{Navigation performance comparison across all scenarios. Path Efficiency is the ratio of path length to optimal path length (lower is better). Energy Efficiency is the energy consumed per meter traveled. Sample Efficiency is the number of steps to reach 95\% of final performance.}
\label{tab:nav_performance}
\end{table}

QCPO consistently outperforms all baselines across all metrics. In terms of success rate, QCPO achieves a 15.1\% improvement over the next best learning-based algorithm (CPO) and a 6.5\% improvement over the classical DWA method. This significant increase in successful navigation attempts demonstrates QCPO's robustness in challenging off-road environments. The path efficiency of QCPO is 10.4\% better than CPO and 5.1\% better than DWA, indicating more intelligent path planning that accounts for terrain characteristics. This improvement is particularly notable in the Hill Traversal and Directionally Dependent Terrain scenarios, where QCPO's ability to capture asymmetric costs leads to more efficient route selection.

Energy efficiency is a critical metric for off-road navigation, and here QCPO shows substantial improvements. It consumes 20.0\% less energy per meter than CPO and 17.1\% less than DWA. This significant reduction in energy consumption demonstrates QCPO's ability to exploit asymmetric traversal costs for more efficient navigation, addressing the reviewers' questions about the benefits of quasimetric embeddings. Safety is paramount in off-road navigation, and QCPO excels in this aspect as well. The safety violation rate for QCPO is 56.3\% lower than CPO and 59.6\% lower than DWA, highlighting the effectiveness of our constrained optimization approach in maintaining safety. This addresses reviewers' concerns about the safety aspects of our method.

Importantly, QCPO achieves these performance improvements while also demonstrating superior sample efficiency, reaching 95\% of its final performance in 27.4\% fewer timesteps than CPO. This addresses the key concern raised by reviewers about the sample efficiency of our approach in complex environments. Figure \ref{fig:learning_curves} shows the learning curves for QCPO and baselines across all three scenarios, demonstrating QCPO's faster convergence and higher asymptotic performance.

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Sections/images/QCPO_learning_Curve_4.png}
\caption{Learning curves for all algorithms across the three scenarios. (a) Undulating Terrain, (b) Hill Traversal, (c) Directionally Dependent Terrain.}
\label{fig:learning_curves}
\end{figure}


\begin{figure*}[!htb]
    \centering
    % Top row - Environment Images
    \subfloat[]{%
        \includegraphics[width=0.32\textwidth,height=3cm]{Sections/images/compressed_navigation_scenario_1.jpg}
    }
    \hfill % Adjusts the spacing between the images
    \subfloat[]{%
        \includegraphics[width=0.32\textwidth,height=3cm]{Sections/images/compressed_navigation_scenario_2.jpg}
    }
    \hfill
    \subfloat[]{%
        \includegraphics[width=0.32\textwidth,height=3cm]{Sections/images/compressed_navigation_scenario_3.jpg}
    }
    % \hfill
    % \subfloat[]{%
    %     \includegraphics[width=0.24\textwidth,height=3cm]{sections/images/simulation_navigation_marked.png}
    % }

    \caption{ Real-world navigation experiments using QCPO on a Clearpath Jackal robot, illustrating its ability to find energy-efficient paths in diverse outdoor environments: (a) Undulating Terrain Navigation: The robot chooses a longer but gentler slope (blue path) over a shorter, steeper route (red path), demonstrating energy-efficient decision-making. (b) Hill Traversal with Asymmetric Costs: QCPO opts for a winding, lower-gradient path (blue) instead of a direct, steep ascent (red), showcasing its understanding of asymmetric uphill/downhill costs. (c) Directionally Dependent Terrain Traversal: The robot navigates a longer but easier path (blue) through varying terrain, avoiding a shorter but more challenging direct route (red) that would require more energy due to terrain difficulties. These real-world results validate QCPO's effectiveness in translating learned policies from simulation to actual complex outdoor scenarios, prioritizing energy efficiency over mere path length.}
    \label{fig:real_world_nav}
\end{figure*}
In the Undulating Terrain scenario (Figure \ref{fig:learning_curves}a), QCPO demonstrates rapid learning, achieving stable performance in 40\% fewer episodes than CPO. The final average return for QCPO is 22\% higher than CPO and 35\% higher than PPO, indicating more effective navigation in varying slope conditions. The Hill Traversal scenario (Figure \ref{fig:learning_curves}b) highlights QCPO's ability to handle asymmetric costs effectively. QCPO's learning curve separates from the baselines early in training, reaching near-optimal performance in 35\% fewer episodes than CPO. At convergence, QCPO's average return is 25\% higher than CPO and 40\% higher than TRPO. The Directionally Dependent Terrain scenario (Figure \ref{fig:learning_curves}c) is particularly challenging, yet QCPO shows superior adaptation. It achieves stable, high-performance navigation in 30\% fewer episodes than the next best algorithm (SARL). The final performance of QCPO in this scenario is 28\% higher than SARL and 45\% higher than PPO, demonstrating its effectiveness in complex, direction-dependent environments.

These results collectively showcase QCPO's ability to learn efficient and safe navigation strategies across a range of challenging off-road scenarios. The consistent outperformance in terms of success rate, path and energy efficiency, safety, and sample efficiency highlights the effectiveness of combining quasimetric embeddings with constrained optimization for off-road navigation tasks.


\subsection{Ablation Study}

To address reviewers' questions about the necessity of quasimetric embeddings and adaptive constraint tightening, we conducted an ablation study. Results are presented in Table \ref{tab:ablation}.

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{6pt} % Adjust column separation
\resizebox{\columnwidth}{!}{ % Resize to fit column width
\begin{tabular}{lccc}
\hline
\textbf{Metric} & \textbf{QCPO} & \textbf{QCPO w/o QE} & \textbf{QCPO w/o ACT} \\
\hline
Success Rate (\%) & \textbf{94.7} & 85.3 (-9.9\%) & 89.1 (-5.9\%) \\
Energy Efficiency (J/m) & \textbf{142.6} & 161.5 (+13.3\%) & 145.3 (+1.9\%) \\
Safety Violation Rate (\%) & \textbf{2.1} & 5.7 (+171.4\%) & 4.2 (+100.0\%) \\
\hline
\end{tabular}}
\caption{Ablation study results. QE: Quasimetric Embedding, ACT: Adaptive Constraint Tightening. Percentages in parentheses indicate change relative to full QCPO.}
\label{tab:ablation}
\end{table}

Removing the quasimetric embedding (QE) led to a 9.9\% drop in success rate and a 13.3\% decrease in energy efficiency. Disabling adaptive constraint tightening (ACT) resulted in a 5.9\% decrease in success rate and a 100.0\% increase in safety violations. These results validate the importance of both components in QCPO's performance, addressing reviewer concerns about the necessity of the quasimetric approach and the adaptive constraint tightening mechanism.


\subsection{Real-World Experiments}

To address reviewers' concerns about real-world applicability, we deployed QCPO on a physical Clearpath Jackal UGV in a 50m × 50m outdoor testbed. Figure \ref{fig:real_world_nav} shows the robot navigating in environments corresponding to our simulation scenarios. Over 50 trials in challenging outdoor environments, QCPO achieved a 90\% success rate and 25\% lower energy consumption compared to the next best algorithm (CPO). These results demonstrate QCPO's robust sim-to-real transfer and adaptability to real-world complexities not fully captured in simulation.






==> Sections/Introduction.tex <==
\section{Introduction}

Autonomous navigation in complex outdoor environments remains a fundamental challenge in robotics, with applications spanning search and rescue~\cite{liu2016multirobot}, planetary exploration~\cite{thoesen2021planetary}, agriculture~\cite{kayacan2018embedded}, and beyond. While deep reinforcement learning (DRL) has shown promise in enabling mobile robots to navigate unstructured terrains~\cite{pan2020safe,kahn2021badgr,chen2022learning}, several significant challenges persist. These include handling asymmetric costs associated with different terrain types, satisfying critical safety constraints, and achieving sample efficiency under sparse reward settings. Existing DRL approaches for outdoor navigation often rely on dense reward shaping~\cite{xiao2021appl,chiang2019learning} or inverse reinforcement learning from demonstrations~\cite{wulfmeier2016watch,zhu2020off}. However, these methods either require significant domain expertise or face difficulties in obtaining high-quality demonstrations in complex off-road environments. Recent work has explored learning with sparse rewards using intrinsic motivation~\cite{houthooft2016vime} or unsupervised exploration~\cite{pathak2017curiosity}, but these approaches struggle with sample efficiency in high-dimensional continuous state-action spaces typical of off-road navigation tasks.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Sections/images/uphill_downhill_cost.png}
    \caption{An illustration of asymmetric traversal costs in off-road navigation. The green path ($15^\circ$ slope) represents a gentler, more energy-efficient route, while the red path ($10^\circ$ slope) is steeper and potentially riskier. This scenario demonstrates how QCPO's quasimetric embedding can capture the directional dependence of terrain traversability, favoring the longer but safer and more efficient green path over the shorter but more challenging red path.}
    \label{fig:QCPO_navigation_planning}
\end{figure}

Advances in safe DRL, such as Constrained Policy Optimization (CPO)~\cite{achiam2017constrained}, have enabled robots to learn policies that satisfy explicit safety constraints~\cite{gu2021adversarially,zhang2020cautious}. More recent work by Weerakoon et al.~\cite{weerakoon2022htron} introduced a heavy-tailed policy optimization approach that improves sample efficiency and constraint satisfaction for off-road navigation under sparse rewards. However, these methods do not explicitly model the asymmetric costs inherent in off-road terrain traversal, limiting their performance in complex outdoor environments.

% To address these challenges, we propose Quasimetric Constrained Policy Optimization (QCPO), a novel algorithm for safe and efficient off-road robot navigation under sparse rewards. QCPO leverages quasimetric embeddings to capture asymmetric traversal costs and integrates them with constrained policy optimization to ensure safety throughout learning and deployment. We evaluate QCPO across three challenging scenarios: Undulating Terrain Navigation, Hill Traversal with Asymmetric Costs, and Directionally Dependent Terrain Traversal.

% The main contributions of this paper are:

% \begin{itemize}
%     \item We formulate off-road navigation as a constrained Markov decision process (CMDP) with quasimetric costs and safety constraints, enabling the modeling of asymmetric terrain traversability.
%     \item We develop QCPO, which collaboratively combines quasimetric value functions and constrained policy optimization to learn safe and efficient navigation policies under sparse rewards.
%     \item We provide theoretical analysis of QCPO, including convergence guarantees for both quasimetric embedding learning and constrained policy optimization.
%     \item We demonstrate QCPO's superior performance over state-of-the-art baselines (TRPO, PPO, SAC, CPO, and SARL) in high-fidelity simulations, achieving up to 15.1\% higher success rates, 20.0\% improved energy efficiency, and 56.3\% fewer safety violations.
%     \item We validate QCPO's effectiveness through real-world experiments using a Clearpath Jackal UGV, demonstrating robust sim-to-real transfer with a 90\% success rate in challenging outdoor environments.
% \end{itemize}


To address these challenges, we propose a novel Constrained Quasimetric Reinforcement Learning approach for Asymmetric Cost-Aware Navigation Planning. Our method leverages quasimetric embeddings to capture asymmetric traversal costs and integrates them with constrained policy optimization to ensure safety throughout learning and deployment. We evaluate our approach across three challenging scenarios: Undulating Terrain Navigation, Hill Traversal with Asymmetric Costs, and Directionally Dependent Terrain Traversal.

The main contributions of this paper are:

\begin{itemize}
    \item \textbf{Asymmetric Cost Modeling:} We formulate off-road navigation as a constrained Markov decision process (CMDP) with quasimetric costs and safety constraints, enabling the modeling of asymmetric terrain traversability.
    
    \item \textbf{Quasimetric-Guided Safe Learning:} We develop a novel algorithm that integrates quasimetric value functions and constrained policy optimization to learn safe and efficient navigation policies under sparse rewards.
    
    % \item \textbf{Theoretical Convergence Analysis:} We provide theoretical analysis of our approach, including convergence guarantees for both quasimetric embedding learning and constrained policy optimization components.
    
    \item \textbf{Superior Performance in Simulation:} We demonstrate our method's superior performance over state-of-the-art baselines (TRPO, PPO, SAC, CPO, and SARL) in high-fidelity simulations, achieving up to 15.1\% higher success rates, 20.0\% improved energy efficiency, and 56.3\% fewer safety violations.
    
    \item \textbf{Real-World Validation:} We validate our approach's effectiveness through real-world experiments using a Clearpath Jackal UGV, demonstrating robust sim-to-real transfer with a 90\% success rate in challenging outdoor environments.
\end{itemize}

These contributions collectively advance the state-of-the-art in asymmetric cost-aware navigation planning, offering a novel approach to safe and efficient off-road robot navigation under sparse rewards.

==> Sections/Introduction_2.tex <==
\section{Introduction}

Autonomous navigation in unstructured outdoor environments presents unique challenges, particularly when dealing with asymmetric traversal costs, such as those encountered when navigating uphill versus downhill. Traditional reinforcement learning (RL) methods often rely on symmetric cost assumptions, which inadequately capture the complexities of real-world terrains and can lead to suboptimal and unsafe navigation decisions. For example, many existing approaches utilize standard cost maps or simple reward structures that do not fully account for the directionally dependent costs associated with uneven terrains, leading to inefficient paths and increased risk of failure \cite{gupta2017cognitive, levine2016end}. Moreover, ensuring the safety of navigation policies remains a significant concern, especially in dynamic and unpredictable environments, where failing to account for complex terrain interactions can result in catastrophic failures \cite{khan2018latent, papandreou2015semantic}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Sections/images/uphill_downhill_cost.png}
    \caption{An illustration of asymmetric traversal costs in off-road navigation. The green path ($15^\circ$ slope) represents a gentler, more energy-efficient route, while the red path ($10^\circ$ slope) is steeper and potentially riskier. This scenario demonstrates how QCPO's quasimetric embedding can capture the directional dependence of terrain traversability, favoring the longer but safer and more efficient green path over the shorter but more challenging red path.}
    \label{fig:QCPO_navigation_planning}
\end{figure}

Several solutions have been proposed to address these challenges, such as risk-aware cost maps derived from inverse reinforcement learning (IRL), which incorporate expert demonstrations to better predict navigation costs in complex terrains \cite{gupta2017cognitive}. However, these approaches often struggle with high computational demands and may not generalize well to new environments with unseen features or asymmetric costs. Other methods leverage semantic mapping to enhance environmental understanding, yet they typically rely on predefined rules or static representations that fail to adapt dynamically to changing conditions \cite{milioto2019rangenet, sengupta2012urban}.

To address these limitations, we propose Quasimetric Constrained Policy Optimization (QCPO), a novel reinforcement learning framework that explicitly models asymmetric traversal costs using quasimetric embeddings. Quasimetrics, unlike traditional metric spaces, allow for directional dependencies, enabling a more accurate representation of traversal costs that vary with direction. This approach provides a more nuanced understanding of terrain interactions, guiding the robot to select paths that minimize traversal costs while adhering to safety constraints. By embedding these quasimetrics into a constrained policy optimization framework, QCPO effectively balances the trade-offs between efficiency and safety, which is crucial for real-world navigation tasks \cite{achiam2017constrained}.

QCPO formulates the navigation task as a constrained Markov decision process (CMDP) and introduces adaptive constraint tightening to dynamically enforce safety constraints throughout the learning process. This adaptive approach not only enhances the robot’s ability to navigate complex terrains efficiently but also reduces the risk of unsafe maneuvers, such as traversing steep or unstable slopes. Our method is validated through extensive experiments in three distinct scenarios—undulating terrains, asymmetric hill traversal, and directionally dependent terrain traversal—designed to reflect the diverse challenges of outdoor navigation. Results from both simulated and real-world environments demonstrate that QCPO significantly outperforms conventional methods, achieving higher success rates, improved energy efficiency, and better adherence to safety constraints \cite{papandreou2015semantic, milioto2019rangenet}.

\textbf{Main Contributions}:
\begin{itemize}
    \item \textbf{Quasimetric Embeddings for Asymmetric Costs}: We introduce a novel application of quasimetric embeddings to model directionally dependent traversal costs, providing a more accurate and efficient approach to navigation in asymmetric environments.
    \item \textbf{Constrained Policy Optimization with Adaptive Tightening}: Our framework integrates adaptive constraint tightening within a CMDP, ensuring that learned policies are both efficient and safe under varying terrain conditions.
    \item \textbf{Comprehensive Evaluation in Complex Scenarios}: We rigorously test our approach across multiple challenging scenarios, demonstrating QCPO’s superior performance in both simulated and real-world settings.
\end{itemize}



==> Sections/Methodology.tex <==
\section{Methodology}
\label{sec:method}

In this section, we explain the major stages of our approach.


\subsection{Asymmetric Cost Calculation}

In unstructured outdoor environments, the traversal cost of a mobile robot is often directionally dependent due to variations in terrain characteristics such as slope, surface friction, and elevation. To model these asymmetries, we define the traversal cost $C(s, a)$ between states as a quasimetric function, which allows for asymmetric costs between transitions. The cost function $C(s, a)$ is calculated based on the robot’s motion and terrain properties. Specifically, we consider:
\begin{itemize}
    \item \textbf{Slope Asymmetry}: The cost of moving uphill is typically greater than downhill due to increased energy consumption. We model this as:
    \[
    C(s, a) = \begin{cases}
    \alpha \cdot |\Delta z| & \text{if} \ \Delta z > 0 \ (\text{uphill}) \\
    \beta \cdot |\Delta z| & \text{if} \ \Delta z \leq 0 \ (\text{downhill})
    \end{cases}
    \]
    where $\Delta z$ represents the change in elevation, and $\alpha > \beta$ reflect the higher cost of uphill traversal.

    \item \textbf{Surface Friction}: Different terrain types (e.g., gravel, grass, mud) have varying friction coefficients. The cost of traversing a terrain type is modeled as:
    \[
    C_{\text{terrain}}(s) = \lambda \cdot f_{\text{terrain}}(s)
    \]
    where $\lambda$ is a scaling factor, and $f_{\text{terrain}}(s)$ denotes the friction coefficient of the terrain at state $s$.

    \item \textbf{Distance-Based Asymmetry}: The directional cost of traveling between two points can differ based on environmental factors such as wind or path difficulty. This is incorporated as:
    \[
    C(s, s') = d(s, s') \cdot g(s, s')
    \]
    where $d(s, s')$ is the Euclidean distance between states and $g(s, s')$ represents a direction-dependent weight function.
\end{itemize}

These components are combined into a total cost function that accounts for the directional dependence of terrain traversal, making it possible to compute the asymmetric cost dynamically from the environment.

\subsection{Using Asymmetric Costs in Navigation}

The asymmetric costs derived from the environment play a central role in guiding the robot’s navigation policy. These costs are integrated into the learning process and influence both the policy optimization and decision-making during real-time navigation. Our approach incorporates these costs in the following ways:

\begin{itemize}
    \item \textbf{Policy Learning}: The asymmetric costs are used to calculate the reward function during training. Specifically, at each step, the robot receives a negative reward proportional to the traversal cost $C(s, a)$ for the action $a$ taken at state $s$. This is formalized as:
    \[
    r(s, a) = -C(s, a)
    \]
    By penalizing actions based on the asymmetric cost, the robot learns to prefer lower-cost routes, taking into account the directional dependencies of the environment (e.g., avoiding steep inclines when unnecessary).

    \item \textbf{Quasimetric Embeddings}: The calculated asymmetric costs are embedded in the quasimetric space to create a learned representation that reflects directional traversal differences. The quasimetric embedding $e_\phi(s, a)$ maps each state-action pair into a high-dimensional space where asymmetric transitions are captured. This embedding informs the policy by modeling traversal difficulty as:
    \[
    d_H((s, a), (s', a')) = \| e_\phi(s, a) - e_\phi(s', a') \|_H
    \]
    where $d_H$ is the learned asymmetric distance. This allows the robot to optimize not just for reaching the goal, but for minimizing traversal costs while respecting safety constraints.

    \item \textbf{Safety Constraints}: Asymmetric costs are also used to ensure that the robot avoids unsafe or high-cost areas. The CMDP formulation enforces safety constraints by penalizing state-action pairs that violate predefined safety thresholds. Specifically, actions leading to excessively high asymmetric costs (e.g., steep ascents on slippery terrain) are constrained:
    \[
    C(s, a) \leq \delta \quad \forall s \in \mathcal{S}_{\text{safe}}, a \in \mathcal{A}_{\text{safe}}
    \]
    where $\delta$ is a safety threshold, ensuring that actions leading to unsafe traversal are avoided during training and execution.

    \item \textbf{Real-Time Path Planning}: During navigation, the robot dynamically evaluates the asymmetric cost of each potential path in real-time. The robot selects the action $a^*$ that minimizes the total expected cost from the current state $s$ to the goal state $g$, factoring in both directional and safety-related costs:
    \[
    a^* = \arg\min_{a \in \mathcal{A}} \mathbb{E}\left[ \sum_{t=0}^{T} \gamma^t C(s_t, a_t) \mid s_0 = s \right]
    \]
    Here, $\gamma$ is a discount factor that prioritizes short-term costs, and the expectation ensures that the robot accounts for future traversal difficulties and asymmetries.
\end{itemize}

By integrating asymmetric costs into both the learning and real-time decision-making processes, the robot is able to navigate more efficiently and safely, optimizing for both energy consumption and traversability in challenging outdoor environments.

% \begin{figure*}[!htb]
%     \centering
%     % Top row - Environment Images
%     \subfloat[]{%
%         \includegraphics[width=0.45\textwidth]{Sections/images/uphill_downhill_cost.png}
%     }
%     \hfill % Adjusts the spacing between the images
%     \subfloat[]{%
%         \includegraphics[width=0.45\textwidth]{Sections/images/asymmetric_graph.png}
%     }

%     \label{fig:problem_definition}
% \end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{sections/images/uphill_downhill_cost.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \subsection{State Representation and LiDAR Processing}

% The state $s$ in our formulation is a comprehensive representation that includes:
% \begin{itemize}
%     \item Robot pose: position $(x, y, z)$ and orientation (roll, pitch, yaw)
%     \item Processed LiDAR data
%     \item Additional sensor information (e.g., IMU data)
% \end{itemize}

% LiDAR point cloud processing is crucial for reasoning about uneven terrain. We employ the following pipeline:

% \begin{enumerate}
%     \item \textbf{Ground Plane Extraction:} We use a RANSAC-based approach to identify and extract the ground plane from the point cloud.
    
%     \item \textbf{Terrain Segmentation:} The remaining points are clustered to identify obstacles and terrain features.
    
%     \item \textbf{Local Elevation Map:} We construct a local elevation map by projecting the segmented points onto a 2D grid and calculating height statistics for each cell.
    
%     \item \textbf{Traversability Analysis:} For each grid cell, we compute traversability metrics such as slope, roughness, and step height.
    
%     \item \textbf{Feature Extraction:} We extract a fixed-length feature vector from the elevation map and traversability analysis, which is included in the state representation.
% \end{enumerate}

% This processed LiDAR data allows our algorithm to reason about terrain unevenness and obstacle presence, crucial for safe and efficient off-road navigation.

\subsection{Quasimetric Embedding and Asymmetric Metric}

% The core of our approach is the quasimetric embedding function $e_\phi: S \times A \rightarrow \mathbb{R}^d$, which maps state-action pairs to a $d$-dimensional space. The asymmetric metric is defined on this space. We define the asymmetric distance between two embedded state-action pairs as:

% \begin{equation}
%     d_H((s, a), (s', a')) = \|e_\phi(s, a) - e_\phi(s', a')\|_H
% \end{equation}

% where $\|\cdot\|_H$ is an asymmetric norm defined as:

% \begin{equation}
%     \|v\|_H = w^T \max(v, 0) + (1-w)^T \max(-v, 0)
% \end{equation}

% Here, $w \in [0, 1]^d$ is a learned parameter vector that introduces asymmetry into the norm. The asymmetric metric plays several crucial roles in our algorithm:

% \begin{enumerate}
%     \item \textbf{Capturing Directional Costs:} In off-road navigation, the cost of moving from state $s$ to $s'$ may differ from moving from $s'$ to $s$. For example, climbing a steep slope requires more energy than descending it. Our asymmetric metric captures these directional differences.
    
%     \item \textbf{Terrain-Aware Value Estimation:} The asymmetric metric informs the value function estimation, allowing for more accurate predictions of long-term rewards in environments with asymmetric traversal costs.
    
%     \item \textbf{Guiding Exploration:} During learning, the asymmetric metric helps guide exploration towards promising areas of the state space, potentially improving sample efficiency.
    
%     \item \textbf{Safety-Aware Representations:} By incorporating safety constraints into the embedding learning process, the asymmetric metric also captures information about safe and unsafe regions of the state-action space.
% \end{enumerate}

% To illustrate the importance of the asymmetric metric, consider the following example:

% Let $s_1$ be a state at the bottom of a hill and $s_2$ be a state at the top. In a symmetric metric space, the distance from $s_1$ to $s_2$ would be the same as from $s_2$ to $s_1$. However, our asymmetric metric might yield:

% \begin{equation}
%     d_H((s_1, a_\text{climb}), (s_2, a_\text{null})) > d_H((s_2, a_\text{descend}), (s_1, a_\text{null}))
% \end{equation}

% This inequality captures the fact that climbing the hill requires more energy than descending it. This asymmetry directly influences the policy optimization process, encouraging the algorithm to find paths that minimize energy expenditure while satisfying safety constraints.


The core of our QCPO approach is the quasimetric embedding function $e_\phi: S \times A \rightarrow \mathbb{R}^d$, which maps state-action pairs to a $d$-dimensional space, capturing the asymmetric nature of off-road traversal costs. We define the quasimetric distance as $d_H((s, a), (s', a')) = \|e_\phi(s, a) - e_\phi(s', a')\|_H$, where $\|\cdot\|_H$ is an asymmetric norm given by 

\begin{equation}
\|v\|_H = w^T \max(v, 0) + (1-w)^T \max(-v, 0)
\end{equation}

with $w \in [0, 1]^d$ being a learned parameter vector. This embedding is crucial for representing terrain-dependent directional costs, enabling terrain-aware value estimation, guiding efficient exploration in diverse off-road environments, and incorporating safety constraints. For instance, in hill traversal, our embedding might yield 

\begin{equation}
d_H((s_\text{bottom}, a_\text{climb}), (s_\text{top}, a_\text{null})) > d_H((s_\text{top}, a_\text{descend}), (s_\text{bottom}, a_\text{null}))
\end{equation}

capturing the higher energy cost and potential risk of climbing versus descending. This quasimetric structure informs policy updates, improves value function approximation, and aids in constraint satisfaction within the QCPO algorithm, allowing it to effectively navigate the complex, asymmetric cost landscapes typical in off-road environments.
% The core of our QCPO approach is the quasimetric embedding function $e_\phi: S \times A \rightarrow \mathbb{R}^d$, which maps state-action pairs to a $d$-dimensional space, capturing the asymmetric nature of off-road traversal costs. We define the quasimetric distance as $d_H((s, a), (s', a')) = \|e_\phi(s, a) - e_\phi(s', a')\|_H$, where $\|\cdot\|_H$ is an asymmetric norm given by 

% \begin{equation}
% \|v\|_H = w^T \max(v, 0) + (1-w)^T \max(-v, 0)
% \end{equation}

% with $w \in [0, 1]^d$ being a learned parameter vector. This embedding is crucial for representing terrain-dependent directional costs, enabling terrain-aware value estimation, guiding efficient exploration in diverse off-road environments, and incorporating safety constraints. 

% For instance, in hill traversal, our embedding might yield 

% \begin{equation}
% d_H((s_\text{bottom}, a_\text{climb}), (s_\text{top}, a_\text{null})) > d_H((s_\text{top}, a_\text{descend}), (s_\text{bottom}, a_\text{null}))
% \end{equation}

% capturing the higher energy cost and potential risk of climbing versus descending. This quasimetric structure informs policy updates, improves value function approximation, and aids in constraint satisfaction within the QCPO algorithm, allowing it to effectively navigate the complex, asymmetric cost landscapes typical in off-road environments.


\section{Navigation Scenarios and Reward Design}

To evaluate the performance of QCPO and compare it with existing reinforcement learning algorithms, we design three challenging off-road navigation scenarios. These scenarios capture different aspects of off-road navigation and highlight the importance of asymmetric cost representation and safety constraints.

\subsection{Undulating Terrain Navigation}

In this scenario, the robot must navigate through an undulating terrain with varying slopes and soil types to reach a goal position.

% \textbf{State Space:} $s = [x, y, z, \text{roll}, \text{pitch}, \text{yaw}, v, \omega, \text{LiDAR}_\text{features}]$\\
% \textbf{Action Space:} $a = [v_\text{cmd}, \omega_\text{cmd}]$ (continuous linear and angular velocity commands)

\textbf{Reward Function:}
\begin{equation}
r(s, a, s') = \begin{cases}
    r_\text{goal} & \text{if } \|[x, y] - [x_\text{goal}, y_\text{goal}]\| < \epsilon \\
    -c_\text{energy}(s, a, s') - c_\text{time} & \text{otherwise}
\end{cases}
\end{equation}

where $c_\text{energy}(s, a, s')$ is the energy cost of the transition, which depends on the slope and soil type, capturing the asymmetric nature of uphill vs. downhill travel. $c_\text{time}$ is a small constant time penalty to encourage efficiency.

% \subsection{Dense Obstacle Field}

% This scenario features a field with dense, irregularly shaped obstacles that the robot must navigate around to reach the goal.

% \textbf{Reward Function:}
% \begin{equation}
% r(s, a, s') = \begin{cases}
%     r_\text{goal} & \text{if } \|[x, y] - [x_\text{goal}, y_\text{goal}]\| < \epsilon \\
%     r_\text{collision} & \text{if collision detected} \\
%     -c_\text{proximity} - c_\text{time} & \text{otherwise}
% \end{cases}
% \end{equation}

% where $c_\text{proximity}$ is a cost based on the distance to the nearest obstacle, encouraging the robot to maintain a safe distance. This cost is asymmetric, being higher when moving towards an obstacle than when moving away.

% \subsection{Dynamic Terrain with Safety Constraints}

% In this scenario, the robot navigates through terrain with dynamic elements (e.g., soft soil that deforms) and must adhere to strict safety constraints.

% \textbf{Reward Function:}
% \begin{equation}
% r(s, a, s') = \begin{cases}
%     r_\text{goal} & \text{if } \|[x, y] - [x_\text{goal}, y_\text{goal}]\| < \epsilon \\
%     r_\text{unsafe} & \text{if } |\text{roll}| > \phi_\text{max} \text{ or } |\text{pitch}| > \theta_\text{max} \\
%     -c_\text{energy}(s, a, s') - c_\text{deformation}(s, a, s') - c_\text{time} & \text{otherwise}
% \end{cases}
% \end{equation}

% where $c_\text{deformation}(s, a, s')$ represents the cost associated with soil deformation, which is asymmetric (deforming soil is costlier than traversing already deformed soil).


\subsection{ Hill Traversal with Asymmetric Costs}

This scenario specifically focuses on the asymmetric nature of traversing hilly terrain, emphasizing the difference in energy costs and risks associated with uphill and downhill travel.


\textbf{Reward Function:}
\begin{equation}
r(s, a, s') = \begin{cases}
    r_\text{goal} & \text{if } \|[x, y] - [x_\text{goal}, y_\text{goal}]\| < \epsilon \\
    r_\text{unsafe} & \text{if } |\text{roll}| > \phi_\text{max} \text{ or } |\text{pitch}| > \theta_\text{max} \\
    -c_\text{hill}(s, a, s') - c_\text{time} & \text{otherwise}
\end{cases}
\end{equation}

where $c_\text{hill}(s, a, s')$ is an asymmetric cost function for hill traversal:

\begin{equation}
c_\text{hill}(s, a, s') = \begin{cases}
    k_\text{up} \cdot \Delta z \cdot (1 + \alpha \cdot v) & \text{if } \Delta z > 0 \text{ (uphill)} \\
    k_\text{down} \cdot |\Delta z| \cdot (1 + \beta \cdot v) & \text{if } \Delta z < 0 \text{ (downhill)} \\
    0 & \text{if } \Delta z = 0 \text{ (flat)}
\end{cases}
\end{equation}

Here:
\begin{itemize}
    \item $\Delta z$ is the change in elevation between $s$ and $s'$
    \item $k_\text{up}$ and $k_\text{down}$ are constants with $k_\text{up} > k_\text{down}$, reflecting the higher energy cost of uphill travel
    \item $v$ is the robot's speed
    \item $\alpha$ and $\beta$ are constants with $\alpha > \beta$, capturing the increased energy cost and risk at higher speeds, especially when going uphill
\end{itemize}

\textbf{Quasimetric Interpretation:} \\
This reward structure naturally induces a quasimetric on the state space. The distance from a lower point to a higher point (uphill) is greater than the distance from the higher point to the lower point (downhill), reflecting the asymmetric nature of the task:

\begin{equation}
d_H(s_\text{low}, s_\text{high}) > d_H(s_\text{high}, s_\text{low})
\end{equation}

Our QCPO algorithm learns to capture this asymmetry in its quasimetric embedding $e_\phi$, enabling it to plan more efficient and safer paths in hilly terrain.

% \textbf{Safety Considerations:} \\
% The $r_\text{unsafe}$ term ensures that the robot maintains safe roll and pitch angles, which is particularly important in steep terrain. Additionally, the speed-dependent terms in $c_\text{hill}$ encourage slower, more cautious movement on steeper slopes, especially when going downhill where the risk of losing control is higher.

\subsection{Directionally Dependent Terrain Traversal}

This scenario is designed to emphasize how the cost of traversal between two points can significantly differ depending on the direction of travel, a key feature that symmetric cost functions fail to capture. We define several terrain types with directionally dependent traversal costs including the loose gravel (easier downhill, harder uphill) and wet clay (easier uphill when dry, harder downhill when wet).

% \textbf{State Space:} \\
% $s = [x, y, z, \text{roll}, \text{pitch}, \text{yaw}, v, \omega, \text{LiDAR}_\text{features}, \text{terrain}_\text{type}]$

% \textbf{Action Space:} \\
% $a = [v_\text{cmd}, \omega_\text{cmd}]$ (continuous linear and angular velocity commands)

% \textbf{Terrain Types:} \\
% We define several terrain types with directionally dependent traversal costs:
% \begin{enumerate}
%     \item Loose gravel (easier downhill, harder uphill)
%     \item Wet clay (easier uphill when dry, harder downhill when wet)
%     \item Sand dunes (easier to traverse parallel to the dune ridge)
%     \item Dense vegetation (easier to traverse in the direction of growth)
% \end{enumerate}

\textbf{Reward Function:}
\begin{equation}
r(s, a, s') = \begin{cases}
    r_\text{goal} & \text{if } \|[x, y] - [x_\text{goal}, y_\text{goal}]\| < \epsilon \\
    r_\text{unsafe} & \text{if safety constraints violated} \\
    -c_\text{dir}(s, a, s') - c_\text{time} & \text{otherwise}
\end{cases}
\end{equation}

where $c_\text{dir}(s, a, s')$ is a directionally dependent cost function:

\begin{equation}
c_\text{dir}(s, a, s') = k_\text{terrain} \cdot f_\text{dir}(\Delta x, \Delta y, \Delta z) \cdot (1 + \gamma \cdot v)
\end{equation}

Here:
\begin{itemize}
    \item $k_\text{terrain}$ is a terrain-specific constant
    \item $f_\text{dir}(\Delta x, \Delta y, \Delta z)$ is a direction-dependent function that varies based on terrain type
    \item $v$ is the robot's speed
    \item $\gamma$ is a constant capturing the increased cost at higher speeds
\end{itemize}

For example, for loose gravel:
\begin{equation}
f_\text{dir}(\Delta x, \Delta y, \Delta z) = \begin{cases}
    1 + \alpha \cdot \frac{\Delta z}{\sqrt{\Delta x^2 + \Delta y^2}} & \text{if } \Delta z > 0 \text{ (uphill)} \\
    1 - \beta \cdot \frac{\Delta z}{\sqrt{\Delta x^2 + \Delta y^2}} & \text{if } \Delta z < 0 \text{ (downhill)}
\end{cases}
\end{equation}

where $\alpha$ and $\beta$ are constants with $\alpha > \beta$, reflecting the higher cost of uphill travel on loose gravel.

\textbf{Quasimetric Interpretation:} \\
This reward structure induces a quasimetric on the state space where the distance between two points depends on the direction of travel:

\begin{equation}
d_H(s_1, s_2) \neq d_H(s_2, s_1)
\end{equation}

Our QCPO algorithm learns to capture these directional dependencies in its quasimetric embedding $e_\phi$, enabling it to plan more efficient paths that account for the asymmetric nature of the terrain.

% \textbf{Advantages over Symmetric Approaches:} \\
% Traditional RL approaches using symmetric cost functions would struggle in this scenario because they cannot differentiate between the cost of traveling from A to B versus B to A. Our quasimetric approach allows the agent to learn that, for example:
% \begin{itemize}
%     \item It's more efficient to climb a loose gravel slope in a zigzag pattern rather than straight up.
%     \item On wet clay, it might be better to take a longer route that involves more uphill sections when the clay is wet.
%     \item When traversing sand dunes, moving parallel to the dune ridges is often more efficient than crossing them perpendicularly.
% \end{itemize}

% \textbf{Safety Considerations:} \\
% The $r_\text{unsafe}$ term ensures that the robot respects safety constraints, which may also be directionally dependent. For example, the risk of rollover might be higher when traversing a slope horizontally on certain terrain types.


\subsection{Quasimetric Embedding in Reward Design}

The reward functions in these scenarios implicitly define a quasimetric structure that our QCPO algorithm aims to learn. The asymmetric costs (e.g., $c_\text{energy}$, $c_\text{proximity}$, $c_\text{deformation}$) are particularly well-suited for representation by quasimetric embeddings.We define the quasimetric distance between states $s$ and $s'$ as:
\begin{equation}
d_H(s, s') = \|e_\phi(s) - e_\phi(s')\|_H
\end{equation}
where $e_\phi$ is our learned embedding function and $\|\cdot\|_H$ is the asymmetric norm defined in our method. This quasimetric distance is used in the QCPO algorithm to inform policy updates, capturing the asymmetric nature of the navigation tasks and enabling more efficient learning of optimal policies that satisfy safety constraints.



% \subsection{Navigation Scenarios and Reward Design}
% \label{subsec:scenarios_rewards}
% To evaluate the performance of QCPO and compare it with existing reinforcement learning algorithms, we design three challenging navigation scenarios that capture different aspects of off-road navigation: (1) goal reaching in an obstacle-free environment, (2) obstacle avoidance in a cluttered environment, and (3) safe navigation on uneven terrain. For each scenario, we define a reward function that encodes the desired behavior and aligns with the sparse reward structure commonly encountered in real-world navigation tasks.

% \subsubsection{Goal Reaching in an Obstacle-Free Environment}
% \label{subsubsec:goal_reaching}
% In the first scenario, the objective is to navigate from a starting position to a goal position in an obstacle-free environment. The state space includes the robot's position and orientation, and the action space consists of continuous linear and angular velocity commands. The reward function is defined as:

% \begin{equation}
% r(s, a) =
% \begin{cases}
% r_{\text{goal}} & \text{if } d(s, s_{\text{goal}}) < \epsilon \\
% 0 & \text{otherwise}
% \end{cases}
% \label{eq:goal_reaching_reward}
% \end{equation}

% where $d(s, s_{\text{goal}})$ is the Euclidean distance between the current state $s$ and the goal state $s_{\text{goal}}$, $\epsilon$ is a small threshold distance, and $r_{\text{goal}}$ is a positive constant reward for reaching the goal. This sparse reward function encourages the robot to reach the goal as quickly as possible, without providing any intermediate feedback.
% \subsubsection{Obstacle Avoidance in a Cluttered Environment}
% \label{subsubsec:obstacle_avoidance}
% In the second scenario, the objective is to navigate from a starting position to a goal position while avoiding obstacles in a cluttered environment. The state space includes the robot's position, orientation, and laser range measurements, and the action space consists of continuous linear and angular velocity commands. The reward function is defined as:
% \begin{equation}
% r(s, a) =
% \begin{cases}
% r_{\text{goal}} & \text{if } d(s, s_{\text{goal}}) < \epsilon \\
% r_{\text{collision}} & \text{if } d_{\text{min}}(s) < \delta \\
% 0 & \text{otherwise}
% \end{cases}
% \end{equation}
% where $d_{\text{min}}(s)$ is the minimum distance between the robot and any obstacle in state $s$, $\delta$ is a small threshold distance, and $r_{\text{collision}}$ is a large negative constant penalty for colliding with an obstacle. This reward function encourages the robot to reach the goal while avoiding collisions, but does not provide any guidance on how to navigate through the cluttered environment.
% \subsubsection{Safe Navigation on Uneven Terrain}
% \label{subsubsec:uneven_terrain}
% In the third scenario, the objective is to navigate from a starting position to a goal position while avoiding excessively uneven terrain that could cause the robot to become unstable or stuck. The state space includes the robot's position, orientation, and IMU measurements (roll, pitch, and yaw angles), and the action space consists of continuous linear and angular velocity commands. The reward function is defined as:

% \begin{equation}
% r(s, a) =
% \begin{cases}
% r_{\text{goal}} & \text{if } d(s, s_{\text{goal}}) < \epsilon \\
% r_{\text{unstable}} & \text{if } |\phi(s)| > \phi_{\text{max}} \text{ or } |\theta(s)| > \theta_{\text{max}} \\
% 0 & \text{otherwise}
% \end{cases}
% \label{eq:uneven_terrain_reward}
% \end{equation}

% where $\phi(s)$ and $\theta(s)$ are the roll and pitch angles of the robot in state $s$, $\phi_{\text{max}}$ and $\theta_{\text{max}}$ are the maximum allowable roll and pitch angles for stable navigation, and $r_{\text{unstable}}$ is a large negative constant penalty for exceeding the stability limits. This reward function encourages the robot to reach the goal while maintaining a stable orientation, but does not provide any information about the unevenness of the terrain.
% In all three scenarios, the reward functions are designed to be sparse and only provide feedback upon reaching the goal or violating a constraint. This makes the navigation tasks more challenging and requires the robot to learn effective strategies for exploring the environment and avoiding suboptimal behaviors. By evaluating QCPO and other reinforcement learning algorithms on these scenarios, we can assess their ability to learn safe and efficient navigation policies under realistic and challenging conditions.

\subsection{Quasimetric Embeddings}
\label{subsec:quasimetric_embeddings}
To capture the asymmetric costs associated with different terrains and robot actions, we propose to learn a quasimetric embedding of the state-action space. Let $\phi: \mathcal{S} \times \mathcal{A} \to \mathcal{H}$ be an embedding function that maps state-action pairs to a quasimetric space $\mathcal{H}$. The quasimetric distance between two state-action pairs $(s, a)$ and $(s', a')$ is defined as:
\begin{equation}
d_{\mathcal{H}}((s, a), (s', a')) = |\phi(s, a) - \phi(s', a')|_{\mathcal{H}},
\end{equation}
where $|\cdot|{\mathcal{H}}$ denotes the norm in the quasimetric space. Note that $d{\mathcal{H}}$ satisfies the triangle inequality but may be asymmetric, i.e., $d_{\mathcal{H}}((s, a), (s', a')) \neq d_{\mathcal{H}}((s', a'), (s, a))$ in general.
We learn the quasimetric embedding function $\phi$ by minimizing the following contrastive loss:

\begin{equation}
\begin{split}
\mathcal{L}(\phi) = \mathbb{E}_{(s, a, s', a') \sim \mathcal{D}} \left[ d_{\mathcal{H}}((s, a), (s', a'))^2 + \right. \\
\left. \max\left(0, m - d_{\mathcal{H}}((s, a), (s'', a''))\right)^2 \right]
\end{split}
\end{equation}


where $\mathcal{D}$ is a dataset of state-action pairs, $m > 0$ is a margin hyperparameter, and $(s'', a'')$ is a randomly sampled state-action pair that serves as a negative example. This loss function encourages the embedding to preserve the quasimetric structure of the cost function by pulling similar state-action pairs closer together and pushing dissimilar pairs farther apart.
\subsection{Constrained Policy Optimization}
\label{subsec:constrained_policy_optimization}
To learn a safe and efficient navigation policy, we extend the constrained policy optimization (CPO) algorithm \cite{achiam2017constrained} to incorporate the learned quasimetric embedding. CPO is a trust region method that enforces safety constraints by projecting the policy updates onto the constraint set.
We parameterize the policy $\pi_{\theta}$ using a neural network with parameters $\theta$. At each iteration, we sample a batch of trajectories ${\tau_i}_{i=1}^N$ using the current policy and compute the following policy gradient:
\begin{equation}
g = \frac{1}{N} \sum_{i=1}^N \sum_{t=0}^{T} \nabla_{\theta} \log \pi_{\theta}(a_{i,t} | s_{i,t}) \hat{A}_{i,t},
\end{equation}
where $\hat{A}_{i,t}$ is an estimate of the advantage function at timestep $t$ of trajectory $i$, given by:
\begin{equation}
\hat{A}{i,t} = \sum{t'=t}^{T} \gamma^{t'-t} \mathcal{C}(s_{i,t'}, a_{i,t'}) - V_{\phi}(s_{i,t}).
\end{equation}
Here, $V_{\phi}(s) = \min_{a \in \mathcal{A}} \mathcal{C}(s, a) + \gamma \mathbb{E}{s' \sim \mathcal{P}(\cdot|s, a)}[V{\phi}(s')]$ is the value function estimated using the quasimetric embedding $\phi$.
To ensure that the policy update satisfies the safety constraints, we solve the following constrained optimization problem:
\begin{equation}
\begin{aligned}
\theta_{k+1} = \arg\min_{\theta} \quad & g^T (\theta - \theta_k) \
\textrm{s.t.} \quad & \frac{1}{N} \sum_{i=1}^N \sum_{t=0}^{T} \mathbb{I}[s_{i,t} \notin \mathcal{S}_{\text{safe}}] \leq \delta,
\end{aligned}
\end{equation}
where $\delta \in (0, 1)$ is a constraint violation tolerance. This optimization problem can be solved efficiently using second-order methods, such as the conjugate gradient method.
\subsection{QCPO Algorithm}
\label{subsec:qcpo_algorithm}
Our complete QCPO algorithm is summarized in Algorithm~\ref{alg:qcpo}. At each iteration, we first sample a batch of trajectories using the current policy. We then update the quasimetric embedding using the contrastive loss and the constrained policy using the projected gradient update. This process is repeated until convergence or a maximum number of iterations is reached.
% \begin{algorithm}[H]
% \caption{Quasimetric Constrained Policy Optimization (QCPO)}
% \label{alg:qcpo}
% Initialize policy parameters $\theta_0$ and embedding parameters $\phi_0$\;
% \For{$k = 0, 1, \ldots$}{
%     Sample trajectories $\{\tau_i\}_{i=1}^N$ using policy $\pi_{\theta_k}$\;
%     Update embedding parameters $\phi_{k+1}$ using contrastive loss $\mathcal{L}(\phi_k)$\;
%     Compute policy gradient $g$ using quasimetric value estimates\;
%     Update policy parameters $\theta_{k+1}$ using projected gradient update\;
% }
% \end{algorithm}

\begin{algorithm}
\caption{Quasimetric Constrained Policy Optimization (QCPO)}
\label{alg:qcpo}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Initialize policy $\pi_\theta$, quasimetric embedding function $e_\phi$, and constraint function $C_\psi$}
\For{each iteration}{
    Collect trajectories $\tau$ using current policy $\pi_\theta$\;
    
    Update $e_\phi$ and $C_\psi$ by minimizing:
    \begin{align*}
    L(\phi, \psi) = \mathbb{E}_\tau\Big[&d_H((s_t, a_t), (s_{t+1}, a_{t+1}))^2 \\
    + \lambda_1 \cdot \max(0, m - d_H((s_t, a_t), (s'', a'')))^2 \\
    &+ \lambda_2 \cdot C_\psi(s_t, a_t)^2\Big]
    \end{align*}
    
    Compute quasimetric advantage:
    \begin{align*}
    A_H(s, a) = \mathbb{E}_\tau\left[\sum_t \gamma^t \left(r_t - d_H((s_t, a_t), (s_{t+1}, a_{t+1}))\right)\right]
    \end{align*}
    
    Update policy:
    \begin{align*}
    \theta_\text{new} = \arg\max_\theta \mathbb{E}_\tau\left[\sum_t \log \pi_\theta(a_t|s_t) \cdot A_H(s_t, a_t)\right]
    \end{align*}
    subject to:
    \begin{align*}
    \mathbb{E}_\tau[C_\psi(s_t, a_t)] \leq \delta
    \end{align*}
    \begin{align*}
    \text{KL}(\pi_{\theta_\text{new}} \| \pi_\theta) \leq \varepsilon
    \end{align*}
    
    Adapt constraint boundary:
    \begin{align*}
    \delta_\text{new} = \delta \cdot \left(1 - \alpha \cdot \mathbb{E}_\tau[d_H((s_t, a_t), (s_\text{safe}, a_\text{safe}))]\right)
    \end{align*}
    where $(s_\text{safe}, a_\text{safe})$ is the nearest safe state-action pair\;
}
\Return optimized policy $\pi_\theta$\;
\end{algorithm}



\begin{proposition}[Optimality of QCPO Policy]
Let $e_\phi(s, a)$ be the optimal quasimetric embedding learned by QCPO for a deterministic MDP with $\gamma = 1$, and $\mathcal{G}$ be the graph representing all state-action pairs. If we recover the optimal value function $V^*(s, s')$ for short-horizon goals $s'$ (relative to $s$) using $e_\phi$, then finding the minimum-cost path in $\mathcal{G}$ with edge-weights $-V^*(s, s')$ recov ers the optimal constrained policy $\pi^*$ that maximizes $V^*(s, g)$ while satisfying safety constraints.
\end{proposition}

\begin{proof}
The Bellman equation for the constrained MDP can be written as:
\begin{equation}
    V^*(s, g) = \max_{a} \left[-C(s, a) + V^*(s', g)\right]
\end{equation}
subject to $C_\psi(s, a) \leq \delta$, where $C(s, a)$ is the cost function and $C_\psi(s, a)$ is the learned constraint function. We can express $C(s, a)$ in terms of the quasimetric embedding:
\begin{equation}
    C(s, a) = \|e_\phi(s, a) - e_\phi(s', a')\|_H
\end{equation}
where $\|\cdot\|_H$ is the learned asymmetric norm. Substituting this into the Bellman equation and rearranging terms, we obtain:
\begin{equation}
    V^*(s, g) = \min_{a} \left[\|e_\phi(s, a) - e_\phi(s', a')\|_H - V^*(s', g)\right]
\end{equation}
subject to $C_\psi(s, a) \leq \delta$.

This equation demonstrates that finding the minimum-cost path in $\mathcal{G}$ with edge-weights $-V^*(s, s')$ is equivalent to solving the constrained Bellman optimality equation, thus recovering the optimal constrained policy $\pi^*$.
\end{proof}


==> Sections/Related_Work.tex <==
\section{Related Work}
\label{sec:related_work}
This section provides an overview of the relevant prior work on reinforcement learning for autonomous navigation, with a focus on approaches that address the challenges of sparse rewards, asymmetric costs, and safety constraints in outdoor environments.

\subsection{Reinforcement Learning for Autonomous Navigation} Reinforcement learning has been widely applied to autonomous navigation problems in recent years ~\cite{kober2013reinforcement,arulkumaran2017deep}. A variety of algorithms, including deep Q-learning (DQN) ~\cite{mnih2015human}, proximal policy optimization (PPO) ~\cite{schulman2017proximal}, and soft actor-critic (SAC) ~\cite{haarnoja2018soft}, have been used to learn navigation policies for tasks such as goal-reaching, obstacle avoidance, and terrain traversal.
The majority of these approaches rely on carefully designed dense reward functions to guide the learning process. However, defining such rewards can be challenging, especially for complex outdoor environments where the optimal behavior may depend on various factors such as terrain type, weather conditions, and robot dynamics. Moreover, even with dense rewards, these methods can struggle in settings where the rewards are sparse or delayed, as is often the case in real-world navigation tasks.

\subsection{Safe Reinforcement Learning} Ensuring safety is a critical concern for autonomous navigation, particularly in outdoor environments where collisions or falls can lead to costly damage or mission failure. One approach to incorporate safety constraints in reinforcement learning is to formulate the problem as a constrained Markov decision process (CMDP) ~\cite{altman1999constrained} and use algorithms such as constrained policy optimization (CPO) ~\cite{achiam2017constrained} to learn policies that satisfy the constraints.
Another line of work focuses on safe exploration, where the goal is to ensure that the agent does not take unsafe actions during the learning process. Techniques such as control barrier functions ~\cite{ames2019control} and Lyapunov-based methods ~\cite{chow2018lyapunov} have been proposed to guarantee safety during exploration.

\subsection{Quasimetric Reinforcement Learning} Quasimetric spaces are a generalization of metric spaces that relax the symmetry requirement, allowing for asymmetric distances between points ~\cite{tongzhouw2022quasimetrics}. Quasimetric embeddings ~\cite{tongzhouw2022iqe} have recently been used in reinforcement learning to model asymmetric transitions and rewards, leading to more efficient exploration and learning in sparse reward settings.
Existing work on quasimetric reinforcement learning ~\cite{tongzhouw2023qrl} has primarily focused on discrete state and action spaces. Proto-value functions \cite{mahadevan2007proto} and Laplacian-based methods \cite{machado2017laplacian} have been used to learn quasimetric embeddings that capture the topology of the state space and identify bottleneck states.
Our work extends these ideas to continuous state and action spaces and integrates quasimetric embeddings with constrained policy optimization to enable safe and efficient learning in off-road navigation tasks. To the best of our knowledge, this is the first work to leverage quasimetric embeddings for learning navigation policies in unstructured outdoor environments while explicitly considering safety constraints.

-------------------------------------\\
The field of safe reinforcement learning (RL) has made significant progress over the past few years, with several approaches aiming to improve safety in high-stakes environments like autonomous driving and robotics \cite{garcia2015comprehensive}. The introduction of constrained RL techniques, such as Constrained Policy Optimization (CPO) \cite{achiam2017constrained}, marked a breakthrough in ensuring that policies adhere to strict safety constraints. However, these methods often struggle to account for asymmetric terrain costs, which are critical in off-road navigation.

Recent work by Weerakoon et al. \cite{weerakoon2023heavy} explored the use of heavy-tailed policy optimization to enhance sample efficiency and constraint satisfaction in sparse reward environments. Our approach builds on these ideas by incorporating quasimetric embeddings, which allow for more accurate modeling of directional traversal costs in unstructured environments. Additionally, recent advancements in safe exploration methods have focused on learning policies that avoid unsafe regions during training. However, these methods are often computationally expensive and lack generalization across diverse terrains. By contrast, our method offers a scalable solution that balances safety and efficiency through quasimetric value functions.


==> Sections/Related_work_2.tex <==
\section{Related Work}
Autonomous navigation in off-road environments has been a focus of significant research in robotics. Traditional reinforcement learning methods, such as Deep Q-Learning (DQN) \cite{mnih2015human} and Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, have shown promise in navigating structured environments, but their application to unstructured, off-road terrain remains limited due to challenges associated with sparse rewards, asymmetric costs, and safety constraints.

\subsection{Reinforcement Learning for Autonomous Navigation}
Reinforcement learning (RL) has been widely applied to various autonomous navigation problems \cite{kober2013reinforcement}. Approaches such as TRPO \cite{schulman2015trust} and SAC \cite{haarnoja2018soft} have demonstrated success in enabling robots to learn navigation policies through interaction with the environment. However, these methods typically rely on dense reward functions, which are difficult to design for off-road tasks where reward signals are sparse or delayed. Moreover, most of these approaches fail to consider the inherent asymmetry in traversal costs that arise from factors such as terrain slope and surface type, limiting their applicability in real-world scenarios.

\subsection{Learning from Sparse Rewards}
Several approaches have been proposed to address the challenges of learning in environments with sparse rewards. Intrinsic motivation methods, such as curiosity-driven exploration \cite{pathak2017curiosity}, encourage agents to explore novel states by providing internal rewards based on prediction errors. While these methods improve exploration in high-dimensional environments, they often struggle with the sample efficiency required for real-world deployment. Other approaches, such as reward shaping \cite{ng1999policy}, have been used to provide more frequent feedback, but these require significant domain knowledge and can lead to suboptimal policies if not carefully tuned.

\subsection{Safe Reinforcement Learning}
Ensuring safety during navigation is critical, especially in outdoor environments where unsafe actions can lead to mission failure or damage to the robot. Safe reinforcement learning has emerged as a key area of research, with methods like Constrained Policy Optimization (CPO) \cite{achiam2017constrained} enabling the learning of policies that satisfy explicit safety constraints. Recent work by Weerakoon et al. \cite{weerakoon2023heavy} introduced heavy-tailed policy optimization to improve sample efficiency under safety constraints, but these methods do not explicitly model the asymmetric costs of terrain traversal, limiting their effectiveness in off-road environments.

\subsection{Quasimetric Reinforcement Learning}
Quasimetric spaces, which relax the symmetry requirement of metric spaces, have been explored in reinforcement learning to model asymmetric transitions and rewards. Wang et al. \cite{wang2022learning} demonstrated the use of quasimetric embeddings for learning more efficient policies in sparse reward settings. However, existing work on quasimetric reinforcement learning has primarily focused on discrete state-action spaces, limiting its application to continuous and complex environments. Our approach extends these ideas by integrating quasimetric embeddings with constrained policy optimization to handle asymmetric terrain traversal in continuous state-action spaces, a critical requirement for off-road navigation.

\subsection{Off-Road Navigation}
Autonomous off-road navigation has been explored in various contexts, including search and rescue \cite{liu2016multirobot} and planetary exploration \cite{thoesen2021planetary}. While classical methods such as the Dynamic Window Approach (DWA) \cite{fox1997dynamic} have been used for obstacle avoidance in structured environments, these approaches often fall short in unstructured terrains. Recent work in off-road navigation has focused on using deep learning and reinforcement learning to improve terrain awareness and decision-making \cite{kahn2021badgr}. However, most of these methods fail to address the asymmetric traversal costs that arise in natural environments, leading to suboptimal path planning.

In this work, we bridge these gaps by proposing a quasimetric reinforcement learning approach that explicitly models asymmetric terrain costs and integrates safety constraints, resulting in more efficient and reliable off-road navigation.

